Diminishing Domain Mismatch for DNN-Based Acoustic Distance Estimation via Stochastic Room Reverberation Models

The room impulse response (RIR) encodes, among others, information about the distance of an acoustic source from the sensors. Deep neural networks (DNNs) have been shown to be able to extract that information for acoustic distance estimation. Since there exists only a very limited amount of annotated data, e.g., RIRs with distance information, training a DNN for acoustic distance estimation has to rely on simulated RIRs, resulting in an unavoidable mismatch to RIRs of real rooms. In this contribution, we show that this mismatch can be reduced by a novel combination of geometric and stochastic modeling of RIRs, resulting in a significantly improved distance estimation accuracy.

==> comparison.tex <==
%% We drop this text and comparision
\begin{figure}[tb]
	\centering
	\resizebox{\linewidth}{!}{
		\input{images/rir_comparison}
	}
   \caption{Comparison of two different simulation approaches for \glspl{RIR} with a recorded \gls{RIR} from MIRaGe. \label{rir_compare} \fromjs{UPDATE picture!}}
\end{figure}
\subsection{Simulation vs.\ Recording}
Fig. \ref{rir_compare} compares two generated \glspl{RIR} (top: PRA cardioid, center: proposed combination of PRA and stochastic model) with a recorded \gls{RIR} from the MIRaGe data set for $T_{60}=0.3s$ and $d=3.12m$.
As mentioned before the \gls{RIR} simulated with PRA is sparse compared to the real \gls{RIR}. By design, the first reflections of the simulated \glspl{RIR} are identical, while the late reverberation of the stochastically simulated \gls{RIR} seems to be more similar to the MIRaGe \gls{RIR}. Although not all characteristics of the real \gls{RIR} are present in the stochastic simulation, like the large negative peak that follows the first peak, the stochastic simulation seems to be a step towards the characteristics of the real \gls{RIR}. \fromtgb{Which characteristics are better modeled?}
